Adaptation to Easy Data in Prediction with Limited Advice

We derive an online learning algorithm with improved regret guarantees for `easy' loss sequences. We consider two types of `easiness': (a) stochastic loss sequences and (b) adversarial loss sequences with small effective range of the losses. While a number of algorithms have been proposed for exploiting small effective range in the full information setting, Gerchinovitz and Lattimore [2016] have shown the impossibility of regret scaling with the effective range of the losses in the bandit setting. We show that just one additional observation per round is sufficient to circumvent the impossibility result. The proposed Second Order Difference Adjustments (SODA) algorithm requires no prior knowledge of the effective range of the losses, $\varepsilon$, and achieves an $O(\varepsilon \sqrt{KT \ln K}) + \tilde{O}(\varepsilon K \sqrt[4]{T})$ expected regret guarantee, where $T$ is the time horizon and $K$ is the number of actions. The scaling with the effective loss range is achieved under significantly weaker assumptions than those made by Cesa-Bianchi and Shamir [2018] in an earlier attempt to circumvent the impossibility result. We also provide a regret lower bound of $\Omega(\varepsilon\sqrt{T K})$, which almost matches the upper bound. In addition, we show that in the stochastic setting SODA achieves an $O\left(\sum_{a:\Delta_a>0} \frac{K^3 \varepsilon^2}{\Delta_a}\right)$ pseudo-regret bound that holds simultaneously with the adversarial regret guarantee. In other words, SODA is safe against an unrestricted oblivious adversary and provides improved regret guarantees for at least two different types of `easiness' simultaneously.

==> adaptive.tex <==
% extension to adaptive:

\subsection{Proof of Theorem \ref{adaptive:thm}} \label{adaptive:thm:proof}
This section contains the analysis of SODA without prior knowledge of $\varepsilon$ for adversarial losses. The analysis is similar to the proof of Theorem~\ref{anytime:thm}. We need the following technical lemma, which replaces Lemma~\ref{anytime:technical}.
\begin{lemma}
\label{adaptive:technical}
For $\hat{S}_{t}$ as defined in \eqref{hatS}, we have for any $T > 1$:
\begin{align*}
  \sum_{t=1}^{T}  \hat{S}_{t} \left ( \frac{1}{\sqrt{\hat{S}_{t-1} +1}} - \frac{1}{\sqrt{\hat{S}_{t} +1}} \right ) \leq 1 + 2\sqrt{\hat{S}_{T-1} +1}
\end{align*}
\end{lemma}
 The proof is provided in appendix \ref{adaptive:technical:proof}.
% here was the theorem

\paragraph{Proof of Theorem \ref{adaptive:thm}}  \label{adaptive:analysis}
Note first that SODA with learning rate given by \eqref{learningrateadaptive} only differs from SODA with learning rate given by \eqref{learningrate} in its dependence on the realization of the algorithm's randomness. This means that the analysis in Section~\ref{anytime:thm:proof} up until taking expectations over the randomness still holds, allowing us to start the current analysis from Lemma~\ref{anytime:lemma}, where we refer to the terms as before:
\begin{align}
  -\sum_{t=1}^{T}\est
  				\leq \underbrace{\frac{\ln K}{\eta_{T}} \vphantom{\eta_{T} \sum_{t=1}^{T} \left ( \est \right)^{2}}}_{\mathclap{\text{1\textsuperscript{st}}}}
  					+ \underbrace{\eta_{T} \sum_{t=1}^{T} \left ( \est \right)^{2}}_{\mathclap{\text{2\textsuperscript{nd}} }}
  					- \underbrace{\sum_{t=1}^{T} \E_{a \sim p_{t}} \left [\est \right]}_{\mathclap{\text{3\textsuperscript{rd}} }}
					+ \underbrace{\sum_{t=1}^{T} \left ( \Phi_{t}(\eta_{t+1}) - \Phi_{t}(\eta_{t}) \right)}_{\mathclap{\text{4\textsuperscript{th}}}}.
\end{align}
Here the expectation of the left hand side is the expected regret against arm $a$ and the third term on the right hand side still vanishes in expectation. We consider first the case where the learning rate is given by $\frac{1}{K-1} \sqrt{ \frac{\ln K}{ \hat{S}_{t-1} +1}}$.

The first term becomes:
\begin{align}
  \frac{\ln K }{\eta_{T}} &=  (K-1)\sqrt{(\hat{S}_{T-1} +1)\ln K } 
  \leq (K-1) \sqrt{ \ln K} \sqrt{\varepsilon^{2} (T-1) + 1}. 
  %&\leq \mathcal{O} \left ( \varepsilon (K-1)\sqrt{T \ln K} \right ). 
  \label{first}
\end{align}

The second term becomes:
%\begin{align}
%  \E \left [\eta_{T} S_{T}(a) \right ] &= \frac{\sqrt{\ln K}}{K-1} \E \left [ \frac{S_{T}(a)}{\sqrt{1 + \frac{1}{(K-1)^{2}} \sum_{a} S_{T-1}(a)}} \right ]\nonumber\\
%  &\leq  \sqrt{\ln K}\E \left [ \frac{S_{T} (a)}{\sqrt {\sum_{a} S_{T}(a)}} \right ]
%  \leq \sqrt{\ln K} \E \left [ \sqrt{S_{T}(a)} \right ]
%  \leq \varepsilon (K-1) \sqrt{T\ln K}  . \label{second}
%\end{align}
\begin{align}
  \eta_{T} S_{T}(a) &= \frac{\sqrt{\ln K}}{K-1}  \frac{S_{T}(a)}{\sqrt{1 + \frac{1}{(K-1)^{2}} \sum_{a} S_{T-1}(a)}} \nonumber\\
  &\leq  \sqrt{\ln K} \frac{S_{T} (a)}{\sqrt {\sum_{a} S_{T}(a)}} 
  \leq \sqrt{\ln K} \sqrt{S_{T}(a)}
  \leq \varepsilon (K-1) \sqrt{T\ln K}  . \label{second}
\end{align}

For the fourth term we use the previous result for the potential derivative \eqref{phiDerivative}. Since the learning rate depends on the randomness of the algorithm, we cannot move the integral outside of the expectation as we did in the previous analysis. Instead, we use a trivial bound on the probability $q_{t}^{\eta} \leq 1$, providing us with a weaker bound, which is partially compensated by the inverse linear scaling in $K$ of the adaptive learning rate defined by \eqref{learningrateadaptive}:
\begin{align*}
   \Phi_{t}(\eta_{t+1}) - \Phi_{t} (\eta_t) %&=    - \int_{\eta_{t+1}}^{\eta_{t}} \Phi_{t}' (\eta) d\eta \\
  &=  \int_{\eta_{t+1}}^{\eta_{t}} \E_{a\sim q_{t}^{\eta}} [ S_{t} ]  d\eta \\
  &=  \int_{\eta_{t+1}}^{\eta_{t}} \sum_{a=1}^{K} q_{t}^{\eta}(a) \sum_{i=1}^{t} (K-1)^{2} \mathbbm{1}(B_{i} = a)  \left(\ell_{i}^{B_{i}} - \ell_{i}^{A_{i}} \right )^{2} d\eta \\
  & = \int_{\eta_{t+1}}^{\eta_{t}}  \sum_{i=1}^{t} q_{t}^{\eta}(B_{i}) (K-1)^{2}  \left(\ell_{i}^{B_{i}} - \ell_{i}^{A_{i}} \right )^{2} d\eta \\
  &\leq (K-1)^{2} \hat{S}_{t} \int_{\eta_{t+1}}^{\eta_{t}} \! \! \! d\eta \\
  &= (K-1) \sqrt{\ln K} \hat{S}_{t} \left ( \frac{1}{\sqrt{\hat{S}_{t-1} +1}} - \frac{1}{\sqrt{\hat{S}_{t} +1}} \right ).
\end{align*}
By Lemma~\ref{adaptive:technical} we then have
\begin{align*}
  \sum_{t=1}^{T} \Phi_{t}(\eta_{t+1}) - \Phi_{t} (\eta_t) &\leq\sqrt{\ln K} (K-1) \left ( 1 + 2 \sqrt{\varepsilon^{2} (T-1) +1} \right ), 
 % \leq \mathcal{O} \left ( \varepsilon (K-1)\sqrt{T \ln K} \right ),
\end{align*}
which combined with the bounds for the first and second term (\eqref{first} and \eqref{second} respectively) gives us the desired bound, using $\sqrt{a+b} \leq \sqrt{a} + \sqrt{b}$ for positive $a,b$. Since this bounds $\mathcal{R}_T^a$ for all $a$, it bounds the expected regret.

For the case where the learning rate at $T$ is instead given by $4 \ln K \geq \hat{S}_{t-1} + 1$, the first term is $ \frac{\ln K }{\eta_{T}} = 2 (K-1) \ln K,$ and the second term is
\begin{align*}
    \eta_{T} S_{T}(a)  &= \frac{1}{2(K-1)} S_{T}(a) \leq \frac{K-1}{2}\hat{S}_{T} 
    \leq \frac{K-1}{2}\left (\hat{S}_{T-1} + 1 \right )
    \leq 2(K-1) \ln K.
\end{align*}
Since the learning rate is constant the potential differences vanish, completing the proof.$\hfill \square$
